Combining E-Graphs with Abstract Interpretation

E-graphs are a data structure that compactly represents equivalent expressions. They are constructed via the repeated application of rewrite rules. Often in practical applications, conditional rewrite rules are crucial, but their application requires the detection - at the time the e-graph is being built - that a condition is valid in the domain of application. Detecting condition validity amounts to proving a property of the program. Abstract interpretation is a general method to learn such properties, traditionally used in static analysis tools. We demonstrate that abstract interpretation and e-graph analysis naturally reinforce each other through a tight integration because (i) the e-graph clustering of equivalent expressions induces natural precision refinement of abstractions and (ii) precise abstractions allow the application of deeper rewrite rules (and hence potentially even greater precision). We develop the theory behind this intuition and present an exemplar interval arithmetic implementation, which we apply to the FPBench suite.

==> benchmark_heatmap.tex <==
\begin{tikzpicture}[scale=0.8]
% \fill[green!15] (5.1,3.5) rectangle (8.5,0);	
% \fill[red!15] (5.1,3.5) rectangle (0,7.1);	
	\begin{semilogxaxis}[xlabel=Lower Bound,ylabel=Upper Bound]
\addplot[scatter, only marks, 
        % scatter src=explicit symbolic,
        %nodes near coords*={\Label},
        %visualization depends on={value \thisrow{name} \as \Label}
        ]%
	table[meta=time] {
         lower upper time
% -0.44	0.44    matrixDeterminant
% -1.52	0.63    delta4
% % -17.16	2.19    delta
% 0.77	-0.07   exp1x
% -1.00	-0.77   nonlin2
% 0.01	-1.00   floudas3
% -1.14	1.00    hartman3
% -1.50	0.00    hartman6
% -0.45	0.05    kepler0
% % -0.86	8.50    kepler1
% % -18.44	2.13    kepler2
% -1.00	-0.77   sec4\_45\_example
% 1.00	-1.00   test04\_dqmom9
% -0.99	-1.00   test05\_nonlin1\_44\_\_32\_r4
% 1.00	-1.00   jetEngine
% -0.38	0.16    turbine1
% % 0.01	3.04    turbine2
% -0.17	0.09    turbine3
% -0.39	0.17    carbonGas
% -0.63	0.63    sine
% 0.01	0.06    sqroot
% -0.88	0.88    sineOrder3
%-0.44	0.44
%-1.52	0.63
%0.77	-0.07
%0.04	-0.01
%0.01	-0.01
%0.00	-0.02
%-1.00	-0.77
%0.00	0.00
%0.00	0.00
%0.00	0.00
%0.01	-1.00
%-1.14	1.00
%-1.50	0.00
%-0.45	0.05
%-1.00	-0.77
%0.01	-0.01
%0.07	-0.01
%1.00	-1.00
%-0.99	-1.00
%0.01	-0.04
%-0.02	0.00
%-0.38	0.16
%% 0.01	3.04
%-0.17	0.09
%0.02	-0.02
%0.00	0.02
%-0.39	0.17
%-0.63	0.63
%0.01	0.06
%-0.88	0.88
%-0.03	0.03
0 0 0.1838048
% 0 0 0.1935892
0.3504296378958131 -0.19701278724303445 2.2519841
0.07163260614929322 -0.04067110488074782 5.1428256
0 0 7.428089
49.25041666597388 -0.974585059174632 5.4824357
% 49.250416665973894 -0.9745850591746329 7.125293
0.5999999999999998 -0.6000000000000001 7.244541
0 0 0.0073426
1 -0.7081967213114754 2.8018885
0 0 34.11048
0 -1 3.9862854
0.1999999999999999 -1 0.0219721
0.9997547316477078 0 1.1928904
0.999734810811868 0 2.8366742
1.319202218048474 -0.3650361412009693 9.363078
0.07701081101259799 -0.19264644366618014 8.0556965
0.07104928247273824 -0.060892649080686596 11.892474
% NaN -0.999 4.3718963
1498.2503748129877 -0.9993330000000002 22.591267
% 2251799813685247 -0.33333333333333354 1.7134433
0.9 -0.9090909090909091 12.16373
0 0 12.178896
99998.99999934493 -0.99999 12.2154255
0.13281682346430557 -0.1161103047895497 6.0582275
0.022982635342185895 0 0.66008747
  };

\end{semilogxaxis}

\end{tikzpicture}


 
 



==> heatmap_naive.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{semilogxaxis}[
    enlargelimits=false,
    colorbar,
    xlabel=Relative Lower Bound,ylabel= Relative Upper Bound
]
\addplot+[scatter,only marks,point meta=explicit]
table[x=lower,y=upper,meta=time]
{
lower upper time name
0 0 0.1881036 matrixDeterminant
0 0 0.220509 matrixDeterminant2
0.24810934430459725 -0.1313418581620233 0.6590594 delta4
0.03581630307464654 -0.020335552440373973 1.5871973 delta
0 0 2.1029932 sqrt_add
0.005008333319484929 0 1.1786251 exp1x
0.005008333319440744 0 1.3643384 exp1x_log
0.5999999999999998 -0.6000000000000001 1.4328603 x_by_xy
1 0 0.5666647 sum
% NaN -0.999 0.8706814 nonlin1
1498.2503748129877 -0.9993330000000002 8.458141 nonlin2
% NaN NaN 0.0088554 i4
0 0 0.0093133 i6
1 -0.7081967213114754 0.4327753 himmilbeau
0 0 4.2474427 azimuth
0 -1 1.9957458 floudas1
0.1999999999999999 -1 0.0210199 floudas3
0.9997547316477078 0 1.1770287 hartman3
0.999734810811868 0 6.4649014 hartman6
0.5276808872193902 -0.11813467352782192 1.0422285 kepler0
0.054292621763881395 -0.16693799277831875 2.3701959 kepler1
0.07104928247273824 -0.060892649080686596 4.155351 kepler2
% NaN -0.999 0.9718775 intro_example
1498.2503748129877 -0.9993330000000002 9.912892 sec4_example
1 0 0.6564889 test01_sum3
0 0 1.4965074 test03_nonlin2
0 0 5.126627 test04_dqmom9
% 99998.99999934493 -0.99999 4.798032 test05_nonlin1,r4
0.13281682346430557 -0.1161103047895497 5.815692 doppler1
0.022982635342185895 0 0.2485796 rigidBody2
0 0 6.3964643 turbine1
0.0069155750156720975 -0.8041785878240878 3.6681645 turbine2
0 0 7.2077913 turbine3
0.16528925619834575 -0.14184397163120585 3.3578088 verhulst
0 0 3.053023 predatorPrey
0 -0.4191865703953882 0.952003 carbonGas
0.2827499937523457 -0.28274999374976323 9.228019 sine
0.1962616822429913 -0.040000000000000265 0.2073037 sqroot
0.35080939134924677 -0.35080939134924677 0.0276835 sineOrder3
0.010362971081844932 -0.00966206233971283 6.3381243 triangle
499.00000000000006 -0.998 1.1972712 intro-example-mixed
};
\end{semilogxaxis}
\end{tikzpicture}
